Proofs and Performance Evaluation of Greedy Multi-Channel Neighbor Discovery Approaches

The accelerating penetration of physical environments by objects with information processing and wireless communication capabilities requires approaches to find potential communication partners and discover services. In the present work, we focus on passive discovery approaches in multi-channel wireless networks based on overhearing periodic beacon transmissions of neighboring devices which are otherwise agnostic to the discovery process. We propose a family of low-complexity algorithms that generate listening schedules guaranteed to discover all neighbors. The presented approaches simultaneously depending on the beacon periods optimize the worst case discovery time, the mean discovery time, and the mean number of neighbors discovered until any arbitrary in time. The presented algorithms are fully compatible with technologies such as IEEE 802.11 and IEEE 802.15.4. Complementing the proposed low-complexity algorithms, we formulate the problem of computing discovery schedules that minimize the mean discovery time for arbitrary beacon periods as an integer linear problem. We study the performance of the proposed approaches analytically, by means of numerical experiments, and by extensively simulating them under realistic conditions. We observe that the generated listening schedules significantly - by up to factor 4 for the mean discovery time, and by up to 300% for the mean number of neighbors discovered until each point in time - outperform the Passive Scan, a discovery approach defined in the IEEE 802.15.4 standard. Based on the gained insights, we discuss how the selection of the beacon periods influences the efficiency of the discovery process, and provide recommendations for the design of systems and protocols.

==> packages/config.tex <==
%!TEX root = ../techreport.tex


\usepackage[utf8]{inputenc}
%\usepackage[T1]{fontenc}
%\usepackage{tabularx}
%\usepackage{multicol}
%\usepackage{graphicx}

\usepackage{tikz}
\usepackage{lipsum}

\usepackage[headsepline,plainheadsepline,footsepline,plainfootsepline]{scrpage2}


\usepackage{mathptmx}
\usepackage[scaled=.92]{helvet}
\usepackage{courier}

% ================================================================
% FIXME package setup
% ================================================================
\usepackage[multiuser,nomargin,marginclue,footnote]{fixme}
% use different colors for fixme levels
\fxusetheme{color}
\fxsetup{targetlayout=colorcb}
% define authors for fixme
% \FXRegisterAuthor{commnad prefix}{environment prefix}{tag}

% Usage example \mcfatal{Has to be fixed ASAP}
% Usage example \mcerror{Problem}
% Usage example \mcwarning{Possible problem}
% Usage example \mcnote{Comment}
% fixme mode
% change 'draft' to 'final' for final version
\fxsetup{status=final}


% ================================================================
% Page Style
% ================================================================

\usepackage{geometry}
\geometry{a4paper, inner=30mm, outer=25mm, top=40mm, bottom=42mm}


\clearscrheadfoot

\ihead[\Large {\scshape TU Berlin }]{\Large {\scshape TU Berlin }}

\ifoot[{\tiny \begin{minipage}{4.0cm}Copyright at Technische Universität Berlin.\newline All Rights reserved.\end{minipage}}]{{\tiny \begin{minipage}{4.0cm}Copyright at Technische Universität Berlin.\newline All Rights reserved.\end{minipage}}}
\cfoot[\scriptsize \trnumber]{\scriptsize \trnumber}
\ofoot[Page \pagemark]{Page \pagemark}

\pagestyle{scrheadings}

\addtokomafont{pagefoot}{\normalfont}



\bibliographystyle{plain}


==> packages/tr_cover.tex <==
%!TEX root = ../techreport.tex

% ================================================================
% Cover Sheet
% ================================================================
{
\sffamily

\thispagestyle{empty}

\setlength{\tabcolsep}{0pt} % remove indent within cell
\noindent % remove indent before cell
\begin{tabularx}{\columnwidth}{cXc}
  \includegraphics[height=1cm]{packages/TU-Logo-3D-rot.pdf}
  & &
  \includegraphics[height=1cm]{packages/tknlogo.pdf}
  \\
\end{tabularx}
\setlength{\tabcolsep}{6pt} % back to default

\vspace{1.0cm}

\begin{center}
{\huge
\noindent
Technische Universität Berlin

\vspace{0.5cm}

\noindent
Telecommunication Networks Group

\begin{center}
\rule{15.5cm}{0.4pt}
\end{center}
}
\end{center}

\begin{minipage}[][11.0cm][c]{14.5cm}
{\Huge

\begin{center}
\trtitle
\end{center}

\begin{center}
{\LARGE \trauthor} \\
{\Large \tremail}
\end{center}


\begin{center}
Berlin, \trdate
\end{center}


\vspace{0.5cm}

}


\begin{center}
\setlength{\fboxrule}{2pt}\setlength{\fboxsep}{2mm}
\fbox{TKN Technical Report \trnumber}
\end{center}

\end{minipage}

\setlength{\fboxrule}{0.4pt}
\setlength{\fboxsep}{0.4pt}

\begin{center}

  \rule{15.5cm}{0.4pt}

  \vspace{0.5cm}

  {\huge {TKN Technical Reports Series}}

  \vspace{0.5cm}

  {\huge Editor: Prof. Dr.-Ing. Adam Wolisz}

  \vspace{0.5cm}

 \end{center}


}

